Simulating dynamic systems using Linear Time Calculus theories

To appear in Theory and Practice of Logic Programming (TPLP). Dynamic systems play a central role in fields such as planning, verification, and databases. Fragmented throughout these fields, we find a multitude of languages to formally specify dynamic systems and a multitude of systems to reason on such specifications. Often, such systems are bound to one specific language and one specific inference task. It is troublesome that performing several inference tasks on the same knowledge requires translations of your specification to other languages. In this paper we study whether it is possible to perform a broad set of well-studied inference tasks on one specification. More concretely, we extend IDP3 with several inferences from fields concerned with dynamic specifications.

==> 00a-head-online.tex <==
\input{idp-latex-all}
\input{99-extra-commands}


\hyphenation{either Logic-Blox}
\providecommand\AMSLaTeX{AMS\,\LaTeX}
\newcommand\eg{\emph{e.g.}\ }
\newcommand\etc{\emph{etc.}}
\newcommand\bcmdtab{\noindent\bgroup\tabcolsep=0pt%
  \begin{tabular}{@{}p{10pc}@{}p{20pc}@{}}}
\newcommand\ecmdtab{\end{tabular}\egroup}
\newcommand\rch[1]{$\longrightarrow\rlap{$#1$}$\hspace{1em}}
% \newcommand\lra{\ensuremath{\quad\longrigDhtarrow\quad}}

  \title[Simulating Dynamic Systems Using LTC]
        {Simulating Dynamic Systems Using Linear Time Calculus Theories - Online Appendix}

  \author[B. Bogaerts et al.]
         {Bart Bogaerts, Joachim Jansen, Maurice Bruynooghe, \and Broes De Cat, Joost Vennekens, and Marc Denecker \\
         Department of Computer Science, KU Leuven\\
         \email{\{firstname.lastname\}@cs.kuleuven.be}}

\pubyear{2014}
\pagerange{\pageref{firstpage}--\pageref{lastpage}}


\begin{document}

\label{firstpage}

\maketitle


 
